The FLoRA Engine: Using Analytics to Measure and Facilitate Learners' own Regulation Activities

The focus of education is increasingly set on learners' ability to regulate their own learning within technology-enhanced learning environments (TELs). Prior research has shown that self-regulated learning (SRL) leads to better learning performance. However, many learners struggle to self-regulate their learning productively, as they typically need to navigate a myriad of cognitive, metacognitive, and motivational processes that SRL demands. To address these challenges, the FLoRA engine is developed to assist students, workers, and professionals in improving their SRL skills and becoming productive lifelong learners. FLoRA incorporates several learning tools that are grounded in SRL theory and enhanced with learning analytics (LA), aimed at improving learners' mastery of different SRL skills. The engine tracks learners' SRL behaviours during a learning task and provides automated scaffolding to help learners effectively regulate their learning. The main contributions of FLoRA include (1) creating instrumentation tools that unobtrusively collect intensively sampled, fine-grained, and temporally ordered trace data about learners' learning actions, (2) building a trace parser that uses LA and related analytical technique (e.g., process mining) to model and understand learners' SRL processes, and (3) providing a scaffolding module that presents analytics-based adaptive, personalised scaffolds based on students' learning progress. The architecture and implementation of the FLoRA engine are also discussed in this paper.

==> sections/backup/02-background.tex <==
% \section{Background}


% The design of the FLoRA system is grounded in the research on SRL conducted over the past few decades. This includes theoretical models of SRL~\cite{winne1998studying,winne2017cognition,winne2020construct,panadero2017review,zimmerman1989social,zimmerman2000attaining,zimmerman2009self} and empirical studies that examined SRL support using human and digital tutoring~\cite{azevedo2005externally,chi2021translating,nye2014autotutor,du2016modelling,johnson2016face,johnson2018pedagogical,graesser2020learning}, artificial intelligence ~\cite{aleven2002effective,azevedo2013international,biswas2016design,azevedotheories}, the principles of multimedia learning~\cite{bannert2014process,biswas2017data,schunk2018handbook,azevedo2019self,sonnenberg2019using,lajoie2021student}. With the use of SRL scaffolds, FLoRA aims to track and improve students' SRL abilities. The term "scaffolding" refers to the practice of giving a student help when they need it, gradually fading out that help as the student's skills become proficient increasingly~\cite{wood1976role,azevedo2022lessons}. Scaffolding, which provides assistance to students when they cannot complete activities on their own and helps them acquire the background information and expertise they will need to complete future assignments, has been demonstrated to enhance the learning process~\cite{hmelo2006understanding,pea2018social,sharma2007scaffolding}. Scaffolding has to be adaptable so that its diagnostic, calibration and fading can function at peak effectivity~\cite{puntambekar2005tools,azevedo2022lessons}, which requires continuous monitoring of the learner's progress. As the learner gains the required competence, the scaffolds may be gradually faded out ~\cite{molenaar2008attention,belland2013framework,duffy2015motivation}.


% Because existing Technology-Enhanced Learning Environments (TELs) are unable to identify students' SRL processes during learning, they employ uniform scaffolding display timing across all students~\cite{molenaar2012dynamic,mengelkamp2012confidence}. That being the case, there is no more effective strategy for providing useful scaffolding to the students in line with their varying levels of achievement. The Metatutor~\cite{azevedo2011metatutor,azevedo2022lessons} and the Agentive~\cite{molenaar2012dynamic} systems are the only ones that deviate from the norm which apply the adaptive scaffolds. By using these systems, learners' progress on a task is monitored, with individualised scaffolds shown accordingly. Though these systems provide adaptive scaffolding, they are not personalised since they do not take into account each learner's unique SRL progress. Based on richer trace data and machine learning models, the FLoRA system will provide options to detect users' learning processes and tailor scaffoldings for each individual learner.


% The FLoRA system aligns with current trends in TELs including an explosion of adaptive learning systems that tailor their instruction, materials, and feedback according to different learners' needs~\cite{winne2013potentials}. Measurement, collection, analysis, and reporting of data on learners and their surroundings are at the heart of recent developments in the developing discipline of learning analytics, which aims to improve education~\cite{gavsevic2015let}. Learners may benefit from learning analytics in a number of ways, including improved performance forecasting, deeper introspection and awareness, and access to relevant, individualised recommendations, feedback, and pedagogical aids such as scaffolds~\cite{verbert2012dataset,tempelaar2015search}. In spite of this, the learning analytics community is not in agreement on which student behaviours in trace data should be used to evaluate students' progress towards SRL goals~\cite{papamitsiou2014learning}. Comparable to previous breakthroughs in diagnosing learners' present knowledge~\cite{baker2016educational}, some machine learning approaches are employed in the FLoRA platform to drive advancements in measuring students' SRL processes and use this new information to adapt scaffolding to learners' SRL processes.






% These systems provide scaffolds in accordance with students' progress on a task. However, the SRL process of an individual student is not monitored and it stands to reason that the scaffolding is not personalised for each student. 































% Tips

% The FLoRA environment currently supports students’ SRL as they write essays based on multiple source texts, a popular learning task administered in different courses and levels of education. Students working in the FLoRA platform are afforded the opportunity to plan their reading and writing session using the Planner tool; interact with readings by creating highlights, tags and notes using the Annotation tool; review/edit annotations using the Search tool; develop essays using the Essay writing tool. During the task, the environment traces learners’ SRL behaviours and sends prompts (i.e., scaffolds) personalised to each learner’s needs. In this way, the learners are prompted to engage in one or more of the following learning processes that are considered critical for productive SRL: (1) task orientation, (2) reading, (3) monitoring of reading, (4) writing, and (5) monitoring of writing. Each scaffold suggests several learning activities to a student and, based on suggested activities, a student can assemble a new learning plan for the reminder of the learning session.

% The FLoRA platform is designed to help learners at different levels of education develop a repository of self-regulatory learning strategies that they can independently and successfully apply in different learning contexts in the future, as students or professionals. More than 2,500 secondary and higher ed students at 16 institutions worldwide have used the Flora platform so far. The preliminary findings indicate that students who used the FLoRA scaffolds enacted more SRL strategies~\cite{lim2022effects,srivastava2022effects} and developed essays of a higher quality (van der Graaf et al., under review), compared to their peers who did not use the FLoRA scaffolds. Our results showed that personalized scaffolds are effective in 1) encouraging learners to adopt diverse SRL processes, 2) facilitating meaningful reading and writing tactics, and 3) urging and facilitating early engagement in SRL processes (Li et al., uder review). 

% Traces of learners’ interactions within the FLoRA environment are collected unobtrusively, as timestamped navigational logs, keystrokes, and mouse clicks. The rich data gathered by FLoRASuch multi-channel data allow for more nuanced measurement of SRL processes, compared to other data collection methods typically used in this research field, e.g., think-aloud protocols, as documented in our recent study (Fan et al., 2022). can These data can be further analysed to advance scholarly understanding of SRL as a dynamic and complex set of learning processes. For example, in our recent studies, we harnessed the FLoRA trace data gathered by FLoRA to empirically document the theorised relationship between learners’ self-regulatory metacognitive processes and their performance in a writing tasktask (Raković et al., 2022). The paper reporting on this study was the best paper runner-up at a major conference on learning analytics.

% FLoRA is a web-based software, hosted on a cloud server (e.g., AWS EC2). It was built on top of the Moodle Learning Management System that is used at many educational institutions worldwide. As such, FLoRA can be easily accessed via any of the popular web browsers and deployed for use in a classroom or research lab. To get the environment ready to use, educators/researchers would only need to upload the writing task instructions and reading materials. They can also customise the list of tags to accommodate requirements of a writing genre (e.g., argumentative essay or lab report). The FLoRA backend contains several highly scalable and reliable components, including Moodle, Elasticsearch, Redis and Swoole. For this reason, FLoRA has demonstrated stability when a few hundred learners used the tool at the same time.















% \begin{table}[ht]
% % table caption is above the table
% \centering
% \caption{Content of all five scaffolds}
% \label{tab:content_of_scaffolding_example} % Give a unique label
% % For LaTeX tables use
% \renewcommand{\arraystretch}{1.5}
% \begin{tabular}{p{4.9cm} p{5.3cm} p{5.1cm}}
% \hline\noalign{\smallskip}
% \textbf{Targeted perspective and Timing} & \textbf{Prompt message} & \textbf{Learning suggestions} \\
% \noalign{\smallskip}\hline\noalign{\smallskip}
% \textbf{\begin{tabular}[c]{@{}l@{}}Scaffold 1 - Orientation \\ (2nd minute)\end{tabular}} & Accurate understanding of the content and requirements of literacy task is critical. Based on your learning behavior so far, we recommend the following steps: & (a) Use table of contents to get an overview and skim text; (b) Check the essay rubric carefully; (c) Make sure you understand the learning goals and instructions; (d) Process information by taking notes.\\
% \hline
% \textbf{Scaffold 2 - Start reading (7th minute)} & Efficient and high-quality reading of information on different topics in the material is essential. Based on your learning behavior so far, we recommend the following steps: & (a) Note down important information; (b) Select what to read next using the table of contents; (c) Check time and monitor your reading progress; (d) Search for (specific) information.\\
% \hline
% \textbf{Scaffold 3 - Monitor reading (16th minute)} & Make sure you only read task-related pages and think about the relationship between reading and writing is the key to learning success. Based on your learning behavior so far, we recommend the following steps: & (a) Review annotations and check what you have learned so far; (b) Review the learning goals and instructions to focus on relevant content; (c) Check your essay structure to determine what to read next; (d) Check the essay rubric.\\
% \hline
% \textbf{Scaffold 4 - Start writing (21st minute)} & Starting writing early and conscientiously writing a high-quality essay is central to the success of this task. Based on your learning behavior so far, we recommend the following steps: & (a) Check the remaining time for writing; (b) Check and re-read the essay rubric; (c) Draft essay by using your own language and transferring learning to main points; (d) Write the essay with help from notes.\\
% \hline
% \textbf{Scaffold 5 - Monitor writing (35th minute)} & At the end of the task, complete the essay according to the task instructions and rubric to get a high score. Based on your learning behavior so far, we recommend the following steps: & (a) Check the essay rubric to revise your essay; (b) Edit your essay to make sure it's complete; (c) Check the learning goals and instructions to avoid digress; (d) Check the timer to manage your time.\\

% \noalign{\smallskip}\hline
% \end{tabular}
% \end{table}








The FLoRA scaffolding architecture employs a request/response communication model~\cite{oluwatosin2014client}, where the client dispatches a scaffold request encapsulating client parameters (user identification, scaffolding condition, elapsed time) at predetermined scaffold intervals. Subsequently, the scaffolding module conducts an analysis of trace actions, responding with a scaffold imbued with pertinent message text and options. Concurrently, the trace parser module operates on a 30-second cycle, ensuring the continuous updating of action and process labels. With these process labels, the scaffolding module can generate two distinct scaffold types: generalized and personalized.

The generalized scaffold uniformly presents identical messages and options to all students, whereas the personalized scaffold customizes these elements based on the individual student's SRL processes. Figure~\ref{fig:trigger_scaffolding} delineates the triggering mechanisms for both generalized and personalized scaffolds at the two-minute mark. This representation underscores the dependence of the prompting process on three critical factors: the student's progression (time elapsed during the task), study condition (generalized or personalized), and, in the case of personalized scaffolding, the student's identity to authenticate individual behavioral labels.

According to our scaffolding framework (\ref{tab:content_of_scaffolding_example}), Orientation-related scaffolds are activated upon the student reaching the two-minute threshold in the writing activity. For students in the generalized condition, the scaffold content for Orientation (including message text and all four options) is sourced from the database, formatted as a JSON object, and transmitted to the client browser for display. In the context of personalized scaffolds, the module assesses the learner's SRL process concerning Scaffold 1 in Table~\ref{tab:content_of_scaffolding_example} before generating the corresponding message and options. For instance, in Figure~\ref{fig:trigger_scaffolding}, at the two-minute mark, a learner exhibiting adequate engagement (exceeding 15 seconds) with the general instruction page and demonstrating reading behaviors (a sequence categorized as \textit{ORIENTATION - MC.O.1} in the process library, involving "$GENERAL\_INSTRUCTION -> NAVIGATION -> RELEVANT\_READING$"), which causes the deactivation of the option to reorient (i.e., "Check the learning goal and instruction") in the first Personalised scaffold. This leaves the learner with only three options. Should all SRL processes be detected, all options within the scaffold are deactivated, leading to the omission of the entire scaffold. This contrasts with generalised scaffolds, where users receive all scaffolds complete with all options, regardless of their divergent learning behaviors.

% The scaffolding module is central to the FLoRA engine. Its primary role is to generate a prompting message with personalized learning suggestion(s) based on students' learning process. In designing SRL support within the FLoRA engine, we adopted the framework proposed by Azevedo and Jacobson~\cite{azevedo2008advances} to address the important questions of \textit{What}, \textit{When}, \textit{How}, and for \textit{Whom} to scaffold. \textit{What} refers to what to scaffold, processing the content (domain-specific), the learning process (domain-general), or both. \textit{When} refers to when to provide a scaffold. \textit{How} refers to the delivery of the scaffold. \textit{Whom} or \textit{What} refers to the delivery system. Figure~\ref{fig:scaffolds_who_why_how_when} provides more description of how these questions were conceptualised in the design of the FLoRA scaffolding module. 








%Researchers have found that students who are able to effectively regulate their own learning are more likely to succeed academically than their counterparts who have trouble with this skill~\cite{azevedo2008externally,bannert2012supporting,fan2022improving,winne2013learning}. Various approaches have been developed to support students SRL~\cite{van2019cue}. However, despite the abundance of practise and consolidation opportunities provided by educational institutions~\cite{bjork2013self}, students often struggle to self-regulate their learning across a variety of contexts~\cite{azevedo2010measuring,bjork2013self,littlejohn2015designing,winne2010improving}.

%Providing SRL scaffoldings, which can help students build their SRL abilities, is one solution to this problem. A student is considered to be scaffolded when they are given assistance on an as-needed basis in order to significantly support them in completing learning tasks that they are unable to complete on their own~\cite{hmelo2006understanding,sharma2007scaffolding,wood1976role}.

%Scaffolding, as demonstrated by a number of previous studies, has been found to foster self-regulation~\cite{azevedo2008externally,bannert2012supporting,veenman2007assessment}, which in turn boosts learning performance and understanding of SRL~\cite{azevedo2004doesB,azevedo2005adaptive,bannert2013scaffolding}. Students require metacognitive guidance (e.g., getting an orientation, setting goals, and creating a plan) in order to successfully regulate their learning and succeed in their courses. Majority of the SRL scaffoldings, however,  has been generic guidance delivered based on pre-defined rules ~\cite{guo2022using}. These SRL scaffoldings do not take into content the learners own learning trajectory or learning strategies and do not give personalised feedback for learners regarding their own SRL processes while they are learning or completing a task. Additionally, the learning effects and intervention mechanism of individual SRL scaffolds has only been the subject of a small number of empirical investigations (ref, ref).  While there is consensus on the need for scaffolding to promote SRL, there is still lack of clarity about the most effective type of scaffold in terms of supporting SRL processes~\cite{devolder2012supporting}. 


% Figure T.x (to be added) provides more description on how these questions were conceptualised in the design of the FLoRA scaffolding engine. More details and reasoning behind the type of prompts, their timing, purpose, and design aesthetics is explained in (ref: upcoming design paper on scaffolds in Metacognition \& Learning)

%The early version of FLoRA focused specifically towards supporting writing-oriented tasks. Hence, the metacognitive and monitoring support provided is to optimise the learning outcome for this specific context (write a good essay). Additionally, the intention has been to provision and evaluate the effects of both \textit{static} and \textit{adaptive} metacognitive support on learners, and thus, flexibility has been provided for both these scenarios within the FLoRA platform. Table \ref{tab:content_of_scaffolding_example} 



% engage closely to orientation process. The first prompt, for instance, is related to "Orientation" and it offers students three tips for getting a handle on the task that corresponded with specific learning procedures (like GENERAL\_INSTRUCTION) and SRL processes (like MC.O.1, GENERAL\_INSTRUCTION -$>$ NAVIGATION -$>$ RELEVANT\_READING). Our scaffolding engine will display the suggestion to "make sure you understand the learning goals and instructions" if it detects that the learner has not read the instruction page (i.e., no MC.O.1 process and GENERAL\_INSTRUCTION action) within a certain period (i.e., the first five minutes); if the learner has read the page, the suggestion will be hidden. So as to minimise the potential for learning interruption, the initial prompt will not appear if the student has completed all three of the engine's proposed procedures and activities.

%Scaffolding has been shown to be effective in a number of studies, although others have discovered that metacognitive scaffoldings (i.e., prompts) on their own don't seem to help much~\cite{berthold2007learning,moser2017effect,van2020effects}. This debate sheds light on a significant informational void: we don't know under what conditions and in what settings scaffolds improve student learning~\cite{guo2022using}. The lack of appropriate understanding and effective design of SRL scaffoldings in digitally personalised education presents significant obstacles.



%There is a wide variety of scaffolding designs available, which are designed to aid in learners' self-regulation. For example, Web-based educational tools~\cite{dabbagh2005using}, student-created quizzes~\cite{jones2019scaffolding}, data visualisation tools~\cite{azevedo2017using}, and SRL-prompt videos~\cite{wong2021examining} and prompts~\cite{bannert2013scaffolding,srivastava2022effects}. Devolder et al.~\cite{devolder2012supporting} emphasised the affordances of prompts as being superior to those of other types of scaffoldings in terms of their ability to improve learning outcomes. The teachers, instructors, researchers, and even students themselves can provide SRL ideas, learning reminders, and strategy recommendations to students via prompts presented as pop-up windows or messages in their online learning environments. As prompts is one of the most generally used scaffolding format~\cite{guo2022using} and its effectiveness is good~\cite{devolder2012supporting}, the FLoRA LMS takes the form of prompts (pop-up windows). Scaffolds content may be dynamically modified with new information as determined by researchers. Meanwhile, the SRL process is collected by FLoRA LMS by analysing data from instrumentation tools, which then triggers the scaffolding procedure based on the learners' real-time learning data.


%Several pop-up windows recommending SRL tasks were offered to students as scaffolds to be used during the activity. The pop-up time of the scaffolding window may be adjusted according to the duration of the task. In the previous lab studies~\cite{fan2021learning,fan2022towards} that use this FLoRA LMS, the task length is 120 minutes. Five distinct views of learning were addressed by five separate prompts and offered to the learners at different time points: Understand the assignment (5th minute), Start reading (17th minute), Monitoring reading (40th minute), Start writing (52nd minute), and Monitoring writing (88th minute), with each prompt containing three learning suggestions. The details of the five prompts is explained in Table~\ref{tab:content_of_scaffolding_example}. It is possible to adjust the scaffolding popup time in response to a modified job duration. Learners who took time at the start of the task to do things like check the essay rubric or use the table of contents to get an overview of the material (orientation process) performed better than those who did not, so a "Orientation" related scaffolding is designed and the timer is set to go off after five minutes.





%While using the FLoRA LMS, students will be given individualised prompts based on their actions throughout the preliminary stages of the primary tasks. All the actions data is saved as the raw trace data. In order to convert raw trace data (such as a navigation log, mouse clicks, and keystrokes) into usable learning actions (such as checking a rubric or taking notes) and SRL processes (such as orientation, planning, monitoring), a trace parser is integrated into the FLoRA LMS  that includes both an action library and a process library (see appendix). An example of a prompt produced by real-time parsing in the fifth minute of the main activity, as shown in Figure~\ref{fig:trigger_scaffolding}, suggesting students to engage closely to orientation process. The first prompt, for instance, is related to "Orientation" and it offers students three tips for getting a handle on the task that corresponded with specific learning procedures (like GENERAL\_INSTRUCTION) and SRL processes (like MC.O.1, GENERAL\_INSTRUCTION -$>$ NAVIGATION -$>$ RELEVANT\_READING). Our scaffolding engine will display the suggestion to "make sure you understand the learning goals and instructions" if it detects that the learner has not read the instruction page (i.e., no MC.O.1 process and GENERAL\_INSTRUCTION action) within a certain period (i.e., the first five minutes); if the learner has read the page, the suggestion will be hidden. So as to minimise the potential for learning interruption, the initial prompt will not appear if the student has completed all three of the engine's proposed procedures and activities.




% To personalise the prompts, learners in this study had their prompts tailored to their own specific needs by taking into account their behaviours in the earlier part of the main tasks. Figure 2 shows an example of a prompt triggered at the fifth minute of the main task based on real time parsing, requesting the learners to orientate themselves. We developed a trace parser which contains an action library and a process library (see appendix) to parse raw trace data (e.g., navigational log, mouse clicks and keyboard strokes) into learning actions (e.g., check rubric or take notes) and SRL processes (e.g., orientation, planning, monitoring). For example, the first prompt which related to "Orientation" and provided learners with three suggestions to better understand the task (as shown in Table 1) which linked to certain learning actions (e.g., GENERAL\_INSTRUCTION) and SRL processes (e.g., MC.O.1, GENERAL\_INSTRUCTION -> NAVIGATION -> RELEVANT\_READING). If our scaffolding engine finds that the learner has not read the instruction page (i.e., no MC.O.1 process and GENERAL\_INSTRUCTION action) within a certain period (i.e., the first five minutes), then the suggestion "make sure you understand the learning goals and instructions" will pop up; and if the learner has already read the page, then the suggestion will be hidden. If the learner achieved all three suggested processes and actions preset by the engine, the first prompt will not pop up, so as to minimise the disruption to learners’ learning.















%\paragraph{Paragraph} \lipsum[7] % Dummy text
%\paragraph{Paragraph} \lipsum[8] % Dummy text

==> sections/backup/anonymoust.tex <==
@article{fan2021learning,
  title={Learning analytics to reveal links between learning design and self-regulated learning},
  author={Fan, Yizhou and Matcha, Wannisa and Uzir, Nora’ayu Ahmad and Wang, Qiong and Ga{\v{s}}evi{\'c}, Dragan},
  journal={International Journal of Artificial Intelligence in Education},
  volume={31},
  number={4},
  pages={980--1021},
  year={2021},
  publisher={Springer}
}
@inproceedings{fan2021learningB,
  title={A learning analytic approach to unveiling self-regulatory processes in learning tactics},
  author={Fan, Yizhou and Saint, John and Singh, Shaveen and Jovanovic, Jelena and Ga{\v{s}}evi{\'c}, Dragan},
  booktitle={LAK21: 11th international learning analytics and knowledge conference},
  pages={184--195},
  year={2021}
}
@article{fan2022improving,
  title={Improving the measurement of self-regulated learning using multi-channel data},
  author={Fan, Yizhou and Lim, Lyn and van der Graaf, Joep and Kilgour, Jonathan and Rakovi{\'c}, Mladen and Moore, Johanna and Molenaar, Inge and Bannert, Maria and Ga{\v{s}}evi{\'c}, Dragan},
  journal={Metacognition and Learning},
  pages={1--31},
  year={2022},
  publisher={Springer}
}
@article{fan2022towards,
  title={Towards investigating the validity of measurement of self-regulated learning based on trace data},
  author={Fan, Yizhou and van der Graaf, Joep and Lim, Lyn and Rakovi{\'c}, Mladen and Singh, Shaveen and Kilgour, Jonathan and Moore, Johanna and Molenaar, Inge and Bannert, Maria and Ga{\v{s}}evi{\'c}, Dragan},
  journal={Metacognition and Learning},
  pages={1--39},
  year={2022},
  publisher={Springer}
}
@inproceedings{rakovic2022using,
  title={Using Learner Trace Data to Understand Metacognitive Processes in Writing from Multiple Sources},
  author={Rakovic, Mladen and Fan, Yizhou and Van Der Graaf, Joep and Singh, Shaveen and Kilgour, Jonathan and Lim, Lyn and Moore, Johanna and Bannert, Maria and Molenaar, Inge and Gasevic, Dragan},
  booktitle={LAK22: 12th International Learning Analytics and Knowledge Conference},
  pages={130--141},
  year={2022}
}
@inproceedings{van2021instrumentation,
  title={Do instrumentation tools capture self-regulated learning?},
  author={Van Der Graaf, Joep and Lim, Lyn and Fan, Yizhou and Kilgour, Jonathan and Moore, Johanna and Bannert, Maria and Gasevic, Dragan and Molenaar, Inge},
  booktitle={LAK21: 11th international learning analytics and knowledge conference},
  pages={438--448},
  year={2021}
}
@article{van2023design,
  title={How to design and evaluate personalized scaffolds for self-regulated learning},
  author={van der Graaf, Joep and Rakovi{\'c}, Mladen and Fan, Yizhou and Lim, Lyn and Singh, Shaveen and Bannert, Maria and Ga{\v{s}}evi{\'c}, Dragan and Molenaar, Inge},
  journal={Metacognition and Learning},
  pages={1--28},
  year={2023},
  publisher={Springer}
}
@article{lim2023effects,
  title={Effects of real-time analytics-based personalized scaffolds on students’ self-regulated learning},
  author={Lim, Lyn and Bannert, Maria and van der Graaf, Joep and Singh, Shaveen and Fan, Yizhou and Surendrannair, Surya and Rakovic, Mladen and Molenaar, Inge and Moore, Johanna and Ga{\v{s}}evi{\'c}, Dragan},
  journal={Computers in Human Behavior},
  volume={139},
  pages={107547},
  year={2023},
  publisher={Elsevier}
}
@article{van2022dynamics,
  title={The dynamics between self-regulated learning and learning outcomes: An exploratory approach and implications},
  author={van der Graaf, Joep and Lim, Lyn and Fan, Yizhou and Kilgour, Jonathan and Moore, Johanna and Ga{\v{s}}evi{\'c}, Dragan and Bannert, Maria and Molenaar, Inge},
  journal={Metacognition and Learning},
  volume={17},
  number={3},
  pages={745--771},
  year={2022},
  publisher={Springer}
}
@article{lim2021temporal,
  title={Temporal assessment of self-regulated learning by mining students’ think-aloud protocols},
  author={Lim, Lyn and Bannert, Maria and van der Graaf, Joep and Molenaar, Inge and Fan, Yizhou and Kilgour, Jonathan and Moore, Johanna and Ga{\v{s}}evi{\'c}, Dragan},
  journal={Frontiers in Psychology},
  volume={12},
  pages={749749},
  year={2021},
  publisher={Frontiers Media SA}
}
@article{rakovic2023harnessing,
  title={Harnessing the potential of trace data and linguistic analysis to predict learner performance in a multi-text writing task},
  author={Rakovi{\'c}, Mladen and Iqbal, Sehrish and Li, Tongguang and Fan, Yizhou and Singh, Shaveen and Surendrannair, Surya and Kilgour, Jonathan and van Der Graaf, Joep and Lim, Lyn and Molenaar, Inge and others},
  journal={Journal of Computer Assisted Learning},
  volume={39},
  number={3},
  pages={703--718},
  year={2023},
  publisher={Wiley Online Library}
}
@article{fan2023towards,
  title={Towards a fuller picture: Triangulation and integration of the measurement of self-regulated learning based on trace and think aloud data},
  author={Fan, Yizhou and Rakovic, Mladen and van Der Graaf, Joep and Lim, Lyn and Singh, Shaveen and Moore, Johanna and Molenaar, Inge and Bannert, Maria and Ga{\v{s}}evi{\'c}, Dragan},
  journal={Journal of Computer Assisted Learning},
  year={2023},
  publisher={Wiley Online Library}
}
@article{li2023analytics,
  title={Analytics of self-regulated learning scaffolding: effects on learning processes},
  author={Li, Tongguang and Fan, Yizhou and Tan, Yuanru and Wang, Yeyu and Singh, Shaveen and Li, Xinyu and Rakovi{\'c}, Mladen and Van Der Graaf, Joep and Lim, Lyn and Yang, Binrui and others},
  journal={Frontiers in Psychology},
  volume={14},
  year={2023},
  publisher={Frontiers Media SA}
}
@inproceedings{fan2022supporting,
  title={Supporting self-regulated learning with data analytics and artificial intelligence},
  author={Fan, Yizhou and Tsai, Yi-Shan and Li, Tongguang and Singh, Shaveen and Rakovic, Mladen and van der Graaf, Joep and Lim, Lyn and Molenaar, Inge and Bannert, Maria and Moore, Johanna and others},
  booktitle={EARLI Special Interest Group 27},
  year={2022}
}
@inproceedings{li2023learners,
  title={Do Learners Appreciate Adaptivity? An Epistemic Network Analysis of How Learners Perceive Adaptive Scaffolding},
  author={Li, Tongguang and Lin, Jionghao and Iqbal, Sehrish and Swiecki, Zachari and Tsai, Yi-Shan and Fan, Yizhou and Ga{\v{s}}evi{\'c}, Dragan},
  booktitle={International Conference on Quantitative Ethnography},
  pages={3--17},
  year={2023},
  organization={Springer}
}
